Economic impacts of AI-augmented R&D

Since its emergence around 2010, deep learning has rapidly become the most important technique in Artificial Intelligence (AI), producing an array of scientific firsts in areas as diverse as protein folding, drug discovery, integrated chip design, and weather prediction. As more scientists and engineers adopt deep learning, it is important to consider what effect widespread deployment would have on scientific progress and, ultimately, economic growth. We assess this impact by estimating the idea production function for AI in two computer vision tasks that are considered key test-beds for deep learning and show that AI idea production is notably more capital-intensive than traditional R&D. Because increasing the capital-intensity of R&D accelerates the investments that make scientists and engineers more productive, our work suggests that AI-augmented R&D has the potential to speed up technological change and economic growth.

==> Previous tex files/cost-data.tex <==
%\subsection{Comparison with AI expenditure data}

%As an independent verification of our estimates, we consider how predicted factor shares for Computer Vision tasks compares to R\&D expenditure data by firms. To do this, we examine a random sample of five publicly-traded firms primarily engaged in producing deep learning research and consumer goods and calculate their human and computational capital expenditure shares from US Securities and Exchange Commission (SEC) filings. As shown in Figure XX.A, the range of capital shares is wide, but the median is close to our estimated capital cost shares and a number of firms do indeed have capital shares that are as high or higher than our estimates.

%To contextualize this data, Figure XX.B includes expenditure data across R\&D sectors, again sampling a set of five firms and examining their R\&D expenditure data from SEC filings. In our sample, we see that software firms that focus on deep learning research and consumer goods have a median capital share 8 times that of other software firms. This increase is remarkable, given that deep learning was not widely in use for software products as recently as 2010 (\cite{goldfarb2022gpt}). Although other sectors lag IT in their adoption of deep learning, we see the start of an increase in capital intensity. [TODO: Fill in AlphaFold and DL in healthcare firms once you have good data. We can argue that we see a slight increase in capital intensity now but not yet the use of large models. Then bring in AlphaFold as example of what we can expect costs to be.] Although this expenditure exercise only relies on a small sample, it provides further evidence that our estimates of the compute share of deep learning R\&D seem to align with firm-level expenditure data and suggests that firms that adopt deep learning become far more capital-intensive than other firms in the same sector.

